CL2CM: Improving Cross-Lingual Cross-Modal Retrieval via Cross-Lingual Knowledge Transfer

Cross-lingual cross-modal retrieval has garnered increasing attention recently, which aims to achieve the alignment between vision and target language (V-T) without using any annotated V-T data pairs. Current methods employ machine translation (MT) to construct pseudo-parallel data pairs, which are then used to learn a multi-lingual and multi-modal embedding space that aligns visual and target-language representations. However, the large heterogeneous gap between vision and text, along with the noise present in target language translations, poses significant challenges in effectively aligning their representations. To address these challenges, we propose a general framework, Cross-Lingual to Cross-Modal (CL2CM), which improves the alignment between vision and target language using cross-lingual transfer. This approach allows us to fully leverage the merits of multi-lingual pre-trained models (e.g., mBERT) and the benefits of the same modality structure, i.e., smaller gap, to provide reliable and comprehensive semantic correspondence (knowledge) for the cross-modal network. We evaluate our proposed approach on two multilingual image-text datasets, Multi30K and MSCOCO, and one video-text dataset, VATEX. The results clearly demonstrate the effectiveness of our proposed method and its high potential for large-scale retrieval.

==> aaai/fig-ablation-transfer-fashion.tex <==



\begin{figure}[tb!]
\centering
\subfigure[Two-stage CL2CM variants training pipeline]{
\label{variants-a}
\includegraphics[width=0.8\columnwidth]{fig/supp_variants.pdf}
}
\subfigure[Performance comparison of different variants]{
\label{variants-b}
\includegraphics[width=0.8\columnwidth, height=100px]{fig/ablation_transfer_fashion.pdf}
}
\vspace{-4mm}
\caption{
Ablation study to investigate the impact of different CL knowledge transfer approaches on Multi30K. Two-stage CL2CM variants initially train a CL network, followed by knowledge transfer to the CM network. The results indicate that CL knowledge transfer achieves significant performance gains, and the multi-level alignment in stage 2 can further improve the target-language representation learning.
}\label{fig:transfer-knowledge-fashion}
\end{figure}

==> fig-ablation-transfer-fashion.tex <==



\begin{figure}[tb!]
\centering
\subfigure[Two-stage CL2CM variants training pipeline]{
\label{variants-a}
\includegraphics[width=0.8\columnwidth]{fig/supp_variants.pdf}
}
\subfigure[Performance comparison of different variants]{
\label{variants-b}
\includegraphics[width=0.8\columnwidth, height=100px]{fig/ablation_transfer_fashion.pdf}
}
\vspace{-4mm}
\caption{
Ablation study to investigate the impact of different CL knowledge transfer approaches on Multi30K. Two-stage CL2CM variants initially train a CL network, followed by knowledge transfer to the CM network. The results indicate that CL knowledge transfer achieves significant performance gains, and the multi-level alignment in stage 2 can further improve the target-language representation learning.
}\label{fig:transfer-knowledge-fashion}
\end{figure}
